Instructional Text Across Disciplines: A Survey of Representations, Downstream Tasks, and Open Challenges Toward Capable AI Agents

Recent advances in large language models have demonstrated promising capabilities in following simple instructions through instruction tuning. However, real-world tasks often involve complex, multi-step instructions that remain challenging for current NLP systems. Robust understanding of such instructions is essential for deploying LLMs as general-purpose agents that can be programmed in natural language to perform complex, real-world tasks across domains like robotics, business automation, and interactive systems. Despite growing interest in this area, there is a lack of a comprehensive survey that systematically analyzes the landscape of complex instruction understanding and processing. Through a systematic review of the literature, we analyze available resources, representation schemes, and downstream tasks related to instructional text. Our study examines 181 papers, identifying trends, challenges, and opportunities in this emerging field. We provide AI/NLP researchers with essential background knowledge and a unified view of various approaches to complex instruction understanding, bridging gaps between different research directions and highlighting future research opportunities.

==> figures/typology_small.bk.tex <==
\tikzset{%
    parent/.style =          {align=center,text width=2cm,rounded corners=3pt, line width=0.3mm, fill=gray!10,draw=gray!80},
    child/.style =           {align=center,text width=2.3cm,rounded corners=3pt, fill=blue!10,draw=blue!80,line width=0.3mm},
    grandchild/.style =      {align=center,text width=2cm,rounded corners=3pt},
    greatgrandchild/.style = {align=center,text width=1.5cm,rounded corners=3pt},
    greatgrandchild2/.style = {align=center,text width=1.5cm,rounded corners=3pt},    
    referenceblock/.style =  {align=center,text width=1.5cm,rounded corners=2pt},
    data/.style =           {align=center,text width=1.2cm,rounded corners=3pt, fill=paired-light-blue!50,draw=paired-dark-blue!65,line width=0.3mm},   
    data_work/.style =      {align=center, text width=4.4cm,rounded corners=3pt, fill=paired-light-blue!50,draw=blue!0,line width=0.3mm},  
    model/.style =           {align=center,text width=1.2cm,rounded corners=3pt, fill=paired-light-orange!50,draw=paired-dark-orange!65,line width=0.3mm},   
    model_work/.style =      {align=center,text width=4.4cm,rounded corners=3pt, fill=paired-light-orange!50,draw=red!0,line width=0.3mm},    
    model_work2/.style =      {align=center,text width=2.8cm,rounded corners=3pt, fill=paired-light-orange!50,draw=red!0,line width=0.3mm},   
    pretraining/.style =        {align=center,text width=1.2cm,rounded corners=3pt, fill= paired-light-green!50,draw=paired-dark-green!75,line width=0.3mm},   
    pretraining_work/.style =   {align=center,text width=4.4cm,rounded corners=3pt, fill= paired-light-green!50,draw= cyan!0,line width=0.3mm},      
    finetuning/.style =           {align=center,text width=1.2cm,rounded corners=3pt, fill= paired-light-purple!50,draw=paired-dark-purple!75,line width=0.3mm},   
    finetuning_work/.style =      {align=center,text width=4.3cm,rounded corners=3pt, fill= paired-light-purple!50,draw= orange!0,line width=0.3mm},        
    inference/.style =           {align=center,text width=1.2cm,rounded corners=3pt, fill= paired-light-red!35,draw=paired-light-red!90,line width=0.3mm},   
    inference_work/.style =      {align=center,text width=4.3cm,rounded corners=3pt, fill= paired-light-red!35,draw= magenta!0,line width=0.3mm},
    hardware/.style =           {align=center,text width=1.2cm,rounded corners=3pt, fill= paired-light-yellow!35,draw=paired-light-yellow!90,line width=0.3mm},   
    hardware_work/.style =      {align=center,text width=4.3cm,rounded corners=3pt, fill= paired-light-yellow!35,draw= magenta!0,line width=0.3mm},
}

\begin{figure*}[!htb]
    \scriptsize
    \centering
    \resizebox{0.9\textwidth}{!}{%
    \begin{minipage}[b]{0.5\linewidth}
    \centering
    \begin{forest}
        for tree={
            forked edges,
            grow'=0,
            draw,
            rounded corners,
            node options={align=center,},
            text width=2cm,
            s sep=4pt,
            calign=child edge, 
            calign child=(n_children()+1)/2,
            l sep=7.5pt,
        },
        [, phantom
            [Data \S\ref{sec:data}, for tree={ data}
                [Unstructured,  data [\citet{wikihowMultilingualSummary,wikiHowStepInference,DeScript}, data_work]
                ]
                [Task-centric,  data
                    [\citet{FengZK18,ParkM18,ZengTNDLX20}, data_work]
                ]
                [Entity-centric,  data
                    [\citet{OpenPI,openPIv2,proparNaacl2018}, data_work]
                ]
                [Symbolic,  data
                    [\citet{PayanMSNPBRCDN23,WebArena23,ALFRED20}, data_work]
                ]
            ]

            [Grounded Tasks \S\ref{ssec:grounded_tasks}, finetuning
                %[Coding Agent, finetuning
                %    [Adapters~\citep{houlsby2019parameter}; \\ LoRA~\citep{hu2022lora}, finetuning_work]
                %]
                [Dialogue Agent, finetuning
                    [ABCD~\citep{ABCD}; \\ TEACh~\citep{TEACh}, finetuning_work]
                ]
                [Web Agent, finetuning
                    [WebArena~\citep{WebArena23}; \\ Mind2Web~\citep{Mind2Web2023}, finetuning_work]
                ]
                [Navigation Agent,  finetuning
                    [ALFRED~\citep{ALFRED20}; VirtualHome~\citep{VirtualHome}, finetuning_work]
                ]
                [Mobile Agent,  finetuning
                    [Mobile-Env~\citep{DanyangZhang2023_MobileEnv}; \citet{li-etal-2020-mapping}, finetuning_work]
                ]
                %?
                [Robotic Agent,  finetuning
                   [CALVIN~\citep{Mees2021CALVINAB}; ~\citet{TellexKDWBTR11}, finetuning_work]
                ]
                [Game Agent,  finetuning
                    [SmartPlay~\citep{wu2024smartplay}; MineCraft~\citep{jayannavar-etal-2020-learning}, finetuning_work]
                ]
            ]            
        ]
    \end{forest}
    \end{minipage}%
    \hspace*{0.4cm}
    \begin{minipage}[b]{0.5\linewidth}
    \begin{forest}
        for tree={
            forked edges,
            grow'=0,
            draw,
            rounded corners,
            node options={align=center,},
            text width=2cm,
            s sep=4pt,
            calign=edge midpoint,
            l sep=7.5pt,
        },
        [, phantom
            [Ungrounded Tasks \S\ref{ssec:ungr_tasks}, for tree={fill=red!45,model}
                [Summarization, model
                    [
                    \citet{Boni2021HowSummAM,wikihowSummary}, model_work]
                ]
                [Event Alignment, model
                    [DeScript~\citep{DeScript};
                    \citet{DonatelliSBKZK21,WanzareZTP17}, model_work]
                ]
                [Implicity Detection/Correction, model
                    [wikiHowToImprove~\citep{AnthonioBR20};
                    ULN~\citep{FengFLW22};
                    , model_work]        
                ]
                [Entity Tracking, model
                    [\citet{KimS23,SconeLongPL16}, model_work]  
                ]
                [Parsing, model
                    [Process Structure Induction, model, [\citet{zhang-etal-2020-analogous, WuZHSP23}, model_work2]],
                    [Process Structure Extraction, model, [\citet{textMining23,MysoreJKHCSFMO19,jermsurawong-habash-2015-predicting}, model_work2]],
                ]
                [Process/Step Generation, model
                    [\citet{YuanCFGSJXY23,proScript}, model_work]  
                ]
                [Question Answering, model
                    [Reasoning, model, [\citet{tandon-etal-2019-wiqa,ZellersHBFC19}, model_work2]],
                    [Reading Comprehension, model, [\citet{Mcscript,Bolotova-Baranova23}, model_work2]],
                ]
                [Knowledge Acquisition/Mining, model
                    [\citet{JungRKM10,ChuTW17}, model_work] 
                ]
            ]
        ]
    \end{forest}
    \end{minipage}
    }
    \caption{Taxonomy of data representation types and related tasks in complex instructional text literature.}
    \label{fig:typo-instruction}
    \vspace{-0.25cm}
\end{figure*}

==> sections/data_task_relation_dump.tex <==
Additionally, we analyzed the relationship between data representation types and tasks to uncover prevalent patterns and potential gaps, and we mapped the temporal and geographical trends in research output to observe the evolution and global spread of this field. These visualizations collectively provide a detailed overview of the current state and trends in instructional text research, guiding us to identify common practices, emerging topics, and areas needing further exploration.

\begin{figure}[h]
\centering
\includegraphics[width=0.6\textwidth]{figures/task_distribution.png}
\caption{Task Types Distribution}
\label{fig:task-type-dist}
\end{figure}


\toreview{}{
\textbf{Figure \ref{fig:task-type-dist}} presents the distribution of different downstream tasks associated with instructional text. The data categorizes tasks into types such as "Information Extraction", "Grounded Task Execution", and "Summarization". This figure shows that "Information Extraction" is the most common task, followed by "Grounded Task Execution", indicating a strong focus on extracting and utilizing information from instructional texts. This highlights the importance of these tasks in understanding and processing instructional content. The dominance of "Information Extraction" and "Grounded Task Execution" suggests that researchers are primarily concerned with interpreting and executing multi-step instructions, which are essential for applications in robotics, virtual assistants, and educational technologies.}



\begin{figure}[h]
\centering
\includegraphics[width=0.75\textwidth]{figures/data_to_task.png}
\caption{Data-Task Distribution}
\label{fig:data-task-dist}
\end{figure}


\toreview{}{
\textbf{Figure \ref{fig:data-task-dist}} illustrates the distribution of data representations across different tasks. The data highlights that "Task-Centric" data is most frequently used across various tasks, followed by "Unstructured" data. This suggests that structured data formats are prevalent in tasks requiring specific procedural knowledge. The prominence of "Task-Centric" data indicates a trend towards using structured representations to enhance the accuracy and efficiency of task execution and information retrieval. This preference for structured data formats aligns with the need for precise and reliable task execution in various applications, highlighting the importance of developing robust data representation methods for instructional texts.}


\begin{figure}[h]
\centering
\includegraphics[width=0.75\textwidth]{figures/heatmap_data_tasks.png}
\caption{Data-Task Heatmap}
\label{fig:data-task-heatmap}
\end{figure}


\toreview{}{
\textbf{Figure \ref{fig:data-task-heatmap}} is a heatmap that further visualizes the relationship between data representations and tasks. The intensity of the colors indicates the frequency of different data-task combinations. Notably, the combination of "Task-Centric" data with "Grounded Task Execution" tasks is very common, highlighting a key area of focus in instructional text research. This frequent pairing underscores the importance of structured data in accurately executing tasks that require understanding and following detailed instructions. The heatmap also reveals areas where certain data types are underutilized, suggesting potential opportunities for future research to explore the application of these data types in various tasks.}


==> tables/tasks_challenges.tex <==
\begin{table}[t]
  \centering
  \small
  % responsive full-width resize; adjust the fraction if needed
  \resizebox{\textwidth}{!}{
  \begin{tabular}{p{0.24\textwidth} p{0.26\textwidth} p{0.32\textwidth} p{0.16\textwidth}}
    \toprule
    \textbf{Challenge} &
    \textbf{Contexts} &
    \textbf{Impact on conclusions} &
    \textbf{Aspect} \\
    \midrule
    Metric brittleness to paraphrase \& step order &
    Summarization; Generation; Reasoning QA &
    Over-states model–human gap &
    Linguistic \\[3pt]
    
    Implicit information handling &
    Implicit-instruction detection; Entity tracking &
    Models omit necessary steps &
    Linguistic \\
    \midrule
    
    Gold-data scarcity &
    Event alignment; Entity tracking; TOD &
    Limits generalization across domains &
    Data scarcity \\[3pt]
    
    Weak-label noise &
    Event alignment; Entity tracking &
    Progress masked by systematic errors &
    Data noise \\
    \midrule
    
    Grounding-blind evaluation &
    TOD; Web/GUI agents; Navigation &
    Inflated scores for unexecutable plans &
    Grounding \\[3pt]
    
    Simulation–reality transfer gap &
    Robotics; Navigation; Web/GUI agents; Mobile GUI &
    High sim scores don’t predict real performance &
    Grounding \\
    \midrule
    
    Causal / temporal correctness failures &
    Entity tracking; Instruction parsing; Summarization; Generation &
    Seemingly correct output is incoherent &
    Reasoning \\
    \midrule
    
    Human-evaluation bottleneck &
    Generation; Parsing; Grounded tasks &
    Over-reliance on weak automatic metrics &
    Scalability \\[3pt]
    
    Simulator-coupled metrics &
    Robotics; Navigation; Web/GUI agents; Mobile GUI &
    Scores incomparable across studies &
    Scalability \\
    \bottomrule
  \end{tabular}}
  \caption{Cross-cutting evaluation challenges for instructional-text tasks.
           Remedies and emerging solutions are detailed in §\ref{sec:cross-cutting-eval}.}
  \label{tab:cross_challenges}
\end{table}

